Early Spectroscopy and Dense Circumstellar Medium Interaction in SN 2023ixf

We present the optical spectroscopic evolution of SN~2023ixf seen in sub-night cadence spectra from 1.18 to 14 days after explosion. We identify high-ionization emission features, signatures of interaction with material surrounding the progenitor star, that fade over the first 7 days, with rapid evolution between spectra observed within the same night. We compare the emission lines present and their relative strength to those of other supernovae with early interaction, finding a close match to SN~2020pni and SN~2017ahn in the first spectrum and SN~2014G at later epochs. To physically interpret our observations we compare them to CMFGEN models with confined, dense circumstellar material around a red supergiant progenitor from the literature. We find that very few models reproduce the blended \NC{} emission lines observed in the first few spectra and their rapid disappearance thereafter, making this a unique diagnostic. From the best models, we find a mass-loss rate of $10^{-3}-10^{-2}$ \mlunit{}, which far exceeds the mass-loss rate for any steady wind, especially for a red supergiant in the initial mass range of the detected progenitor. These mass-loss rates are, however, similar to rates inferred for other supernovae with early circumstellar interaction. Using the phase when the narrow emission features disappear, we calculate an outer dense radius of circumstellar material $R_\mathrm{CSM, out}\sim5\times10^{14}~\mathrm{cm}$ and a mean circumstellar material density of $\rho=5.6\times10^{-14}~\mathrm{g\,cm^{-3}}$. This is consistent with the lower limit on the outer radius of the circumstellar material we calculate from the peak \Halpha{} emission flux, $R_\text{CSM, out}\gtrsim9\times10^{13}~\mathrm{cm}$.

==> figset_translation_table.tex <==
spectra_montage_2pg_1.pdf & Optical Spectra Day 1-5.2
spectra_montage_2pg_2.pdf & Optical Spectra Day 5.2-14
